Coded Merkle Tree: Solving Data Availability Attacks in Blockchains

In this paper, we propose coded Merkle tree (CMT), a novel hash accumulator that offers a constant-cost protection against data availability attacks in blockchains, even if the majority of the network nodes are malicious. A CMT is constructed using a family of sparse erasure codes on each layer, and is recovered by iteratively applying a peeling-decoding technique that enables a compact proof for data availability attack on any layer. Our algorithm enables any node to verify the full availability of any data block generated by the system by just downloading a $\Theta(1)$ byte block hash commitment and randomly sampling $\Theta(\log b)$ bytes, where $b$ is the size of the data block. With the help of only one connected honest node in the system, our method also allows any node to verify any tampering of the coded Merkle tree by just downloading $\Theta(\log b)$ bytes. We provide a modular library for CMT in Rust and Python and demonstrate its efficacy inside the Parity Bitcoin client.

==> 4_spar_details.tex <==
\vspace{-4mm}
\section{Detailed Description of SPAR}\label{sec:SPAR_details}
\vspace{-3mm}
In this section, we describe the four core components of SPAR: the construction of the coded Merkle tree by the (honest) block producer, the sampling mechanism of the light nodes, the decoding and alerting operations of the honest full nodes, and the erasure codes used by SPAR. At the end of this section, we will summarize the action space of each node in the network.

\vspace{-5mm}

\subsection{Construction of coded Merkle tree}
\label{sec:cmt_construction}
\vspace{-1mm}
In SPAR, an honest full node detects and proves incorrect-coding
using the membership proofs of \emph{all} the $d$ coded symbols in one parity equation and the values of at least $d-1$ of these coded symbols. Since any parity equation can be compromised, a light node needs to make sure the membership proofs of \emph{all} the $n$ coded symbols are available at honest full nodes. In other words, it needs to make sure the entire Merkle tree is available.

To this end, we propose CMT. At a high level, CMT applies erasure coding to every layer of the tree, where the data symbols of a layer are generated using the hashes of the coded symbols of its child layer. This way, a light node can check the availability of every layer through random samplings, whilst an honest full node can detect and prove the incorrect coding at any layer, with the help of the hashes of this layer provided at its parent layer.

More specifically, given a block of $k$ data symbols, a rate-$r$ ($r \leq 1$) systematic erasure code with an undecodable ratio of $\alpha$ is applied to generate $n=k/r$ coded symbols, where the first $k$ are the original data symbols and the remaining $n-k$ are called parity symbols (hence the name systematic). Then the hashes of every $q$ coded symbols are batched as one data symbol for the next (parent) layer. This yields a total of $n/q$ data symbols for the next layer, which will be encoded using a smaller (in terms of $k$) rate-$r$ systematic code with the same undecodable ratio. This iterative encoding and batching process stops once there are only $t$ ($t\geqslant 1$) hashes in a layer. These $t$ hashes are the root of the CMT, and will be included in the block header and published with the original data block.

CMT layer size reduces at a rate of $qr$. Thus, $qr>1$ for CMT to converge.  In addition, to enable efficient sampling of both data and parity symbols (will discuss next), batching is interleaved, namely, the $q$ coded symbols whose hashes are batched together consist of $qr$ data symbols and $q(1-r)$ parity symbols. An example of CMT with $k=16$, $r=\frac{1}{2}$, $q=4$, and $t=4$ is illustrated in Fig.~\ref{fig:coded_Merkle_tree_interleaved}. Indeed, a classic Merkle tree is a special CMT with $r=1$ and $q=2$.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/CMT.png}
    \caption{Coded Merkle tree for $k=16$ data symbols using rate $r=\frac{1}{2}$ erasure codes. Each data symbol of a higher layer is constructed by batching the hashes of $qr=2$ data symbols and $q(1-r)=2$ parity symbols of its child layer.}
    \label{fig:coded_Merkle_tree_interleaved}
    \vspace{-6mm}
\end{figure*}

\vspace{-5mm}

\subsection{Sampling Mechanism of Light Nodes}
\label{sec:samplingalgorithm}

\vspace{-2mm}
In SPAR, a light node randomly samples the base layer coded symbols with their Merkle proofs to decide the availability of the base layer. The special structure of CMT allows them to further utilize these proofs to efficiently sample higher layer symbols to decide the availability of higher layers.

Similar to a classic Merkle tree, the Merkle proof of a base layer symbol in CMT consists of all the sibling hashes between this symbol and the root. The only difference is that the number of sibling hashes per layer is now $q-1$ instead of 1, which effectively provides the light node one data symbol from every intermediate layer. Thus, when a light node randomly samples $s$ distinct base layer coded symbols, the associated Merkle proofs will automatically sample,  at \emph{no} extra cost, $s$ distinct data symbols from every intermediate layer w.h.p.

To properly check the availability of an intermediate layer,
%To achieve uniform sampling on an intermediate layer, 
a light node should also randomly sample about $(1-r)s$ parity symbols from this layer. To avoid downloading extra Merkle proofs for these parity symbols and to minimize the correlation between the samplings\footnote{Otherwise, the malicious block producer can hide the highly correlated symbols of the same layer together to reduce light nodes' detection probability.}, SPAR samples parity symbols of intermediate layers probabilistically: For every pair of parent and child intermediate layer, if a parent layer data symbol is sampled, then with probability $1-r$, one of its $q(1-r)$ child parity symbols (thanks to interleaved batching) will be sampled uniformly at random. %This way, when $s$ data symbols of the parent layer are sampled, an average of $s(1-r)$ parity symbols from the child layer will be sampled. 
Thus, the response size of one sampling request will be:
\vspace{-0.5em}
\begin{equation}\label{eq:merkle_proof_with_parity}
    \frac{b}{k}+\left[y(q-1) + yq(1-r)\right]\log_{qr}\frac{k}{rt},
\vspace{-2mm}
\end{equation}
where $\frac{b}{k}$ is the base layer symbol size, $y$ is the hash  size (e.g., 32 bytes), $y(q-1)$ is the size of the partial data symbol from an intermediate layer for Merkle proof, $yq(1-r)$ is the average size of probabilistically sampled parity symbol from an intermediate layer, and $\log_{qr}\frac{k}{rt}$ is the number of layers. See Fig.~\ref{fig:Merkle_proof} for sampling response of a coded symbol on the based layer of the CMT in Fig.~\ref{fig:coded_Merkle_tree_interleaved}.

Finally, to counter selective disclosure conducted by the malicious block producer, a light node will make the $s$ requests separately, anonymously, with replacement, and with some delay between every two requests. This will prevent the malicious block producer from selectively deceiving any particular light node, or deceiving the set of light nodes that make requests at the beginning. Therefore, every light node will have the same chance to catch data availability attack.
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/Merkle_proof.png}
    \caption{Merkle proof in CMT, and probabilistic sampling of parity symbols in intermediate layers. The solidly circled symbols constitute a base layer coded symbol and its Merkle proof. For the 2 dash-circled yellow parity symbols, with a probability of $1-r=0.5$, one of them (with equal chance) will be included in the proof for sampling purpose. So will the 2 dash-circled blue parity symbols.}
    \label{fig:Merkle_proof}
    \vspace{-6mm}
\end{figure*}

% \begin{algorithm}
% \caption{Coded Merkle Tree Construction} \label{alg:STC0}
% \KwIn{$G_{1},\dots,G_{\ell_{th}},{\bf c}_{0},k,r,q,t$}
% \KwOut{ the coded Merkle tree ${\bf c}_{1},\dots, {\bf c}_{\ell_{th}}$}
% Let $k_0 = k$, $n_0 = k/r$, $\ell = 0$.\\
% \While{$n_\ell > t$}{
% Let ${\bf c}_{\ell} = [c_{\ell,1},\dots,c_{\ell,n_\ell}] =  [c_{\ell,1},\dots,c_{\ell,k_\ell}]G_\ell$.\\
% Let $[h_{\ell,1},\dots,h_{\ell,n_\ell}]$ be the hashes of $[c_{\ell,1},\dots,c_{\ell,n_\ell}]$.\\
% \For{ $i\in [n_\ell /q]$}{
% Let $c_{\ell + 1,i} = [h_{\ell,(i-1)rq+1},\dots,h_{\ell,(i-1)rq + rq },$ \\$h_{\ell, (i-1)(1-r)q + k_\ell + 1},\dots,h_{\ell, (i-1)(1-r)q+ k_\ell + (1-r)q } ]$.}
% Increment $\ell$. Let $k_\ell = n_{\ell-1} /q$, $n_\ell =k_\ell/r$.
% }
% \Return ${\bf c_1},\dots,{\bf c}_{\ell_{th}}$. 
% \end{algorithm}

\vspace{-2em}

\subsection{Hash-aware peeling decoder and incorrect-coding proof}\label{sec:peeling_decoder}
A hash-aware peeling decoder is similar to conventional LDPC peeling decoder. Given the hashes of all the $n$ coded symbols and $(1-\alpha)n$ coded symbols of a layer, it iteratively solves degree-1 parity equations and check each decoded symbol against its hash and associated parity equations (Algorithm \ref{alg:peeling}). This way, the detection and proof of incorrect-coding is minimized to one parity equation.

The key condition for the peeling decoder to work is that the hashes of all the coded symbols are available. This is assured by CMT: By first downloading the root, the decoder will have all the hashes needed to decode the previous layer. Once this layer is successfully decoded, the decoded data symbols will provide all the hashes needed to decode its child layer. This top-down decoding continues until the data block is decoded, or incorrect-coding is detected at one of the layers. To prove a failed parity equation that consists of $d$ coded symbols, the decoder only needs to provide the Merkle proofs of these coded symbols, and the value of $d-1$ coded symbols. Note that the higher the failed layer, the shorter the Merkle proof of each symbol in the incorrect-coding proof.

In addition, the peeling decoder only works if 1) there are $(1-\alpha)n$ coded symbols available, and 2) that these coded symbols allow the recovery of all the $k$ data symbols. While the first condition is checked by light nodes through random sampling, the second condition requires us to find, for every layer, a erasure code whose undecodable ratio is $\alpha$ under peeling decoding. The best performance is achieved if the codes are extremely sparse (with a small $d$) and have a large $\alpha$. We now present such an ensemble of LDPC codes.

% \subsubsection{Proof of poor erasure code.}
% A full node may also detect codes with poor stopping distance, if it receives a substantial portion of the block but cannot proceed with the peeling decoder (line 11 in Algorithm \ref{alg:peeling}). In this case, the full node generates a proof of poor erasure code by sending the indices of the available symbols to the network. Any node in the network can efficiently check that the remaining indices of the code form a stopping set. The network then agree to draw a new erasure code from the ensemble described in Section \ref{sec:erasurecodeconstruction}.


\vspace{-4mm}

\subsection{Construction of Erasure Code}
\label{sec:erasurecodeconstruction}
\vspace{-2mm}
\def\S{\mathcal S}
\def\c{\boldsymbol c}
% As explained, the systematic symbols at each layer of the coded Merkle Tree are encoded with an LDPC code. The sparse parity check matrix allows the full nodes to construct succinct proofs of incorrect coding for the light nodes. However, in order to successfully detect unavailable symbols, a good LDPC code must have a large stopping ratio. This means that the peeling decoder discussed in the previous section must be able to decode an LDPC codeword having access to only a (large) constant fraction of the symbols. This will ensure that a malicious block producer who intends to make the block undecodable will have to hide a constant fraction of the codeword symbols. As a result, a light node will be able to detect the missing symbols with high probability.
An $(n,k)$ erasure code can be described by an $n\times (n-k)$ parity check matrix $\sH$, where each column of $\sH$ describes a parity equation, such that $\sC\sH=\overrightarrow{0}$ for any valid codeword $\sC$. In addition, every \emph{stopping set} of $\sH$ corresponds to a set of coded symbols whose hiding will prevent the full recovery of data symbols using peeling decoder.
%\begin{definition}[Stopping Set]
For an $ n\times (n-k)$ parity check matrix $\sH$, a set of rows $\tau \subset [n]$ is called a {\em stopping set} if no column in $\sH_\tau$ has one non-zero element. Here $\sH_\tau$ is the submatrix of $\sH$ that only consists of the rows in $\tau$.
%\end{definition}

\begin{algorithm}[t]
\caption{Hash-aware peeling decoding algorithm}\label{alg:peeling}
\label{alg:peeling}
{\textbf{Inputs}: the hashes of all $n$ coded symbols and $(1-\alpha)n$ coded symbols;}\\
{\textbf{Initial check}: checks all the degree-0 parity equations (i.e., those whose coded symbols are all known). If any parity equation is failed, report an incorrect-coding proof and exit;}\\
\While{not all the $k$ data symbols are recovered}{
Find a degree-1 parity equation, which only has one unknown coded symbol;\\
Recover this coded symbol and verify it with its hash. If failed, report an incorrect-coding proof and exit;\\
Check all the associated degree-0 parity equations. If any parity equation is failed, report an incorrect-coding proof and exit.}
\end{algorithm}

%\vspace{-20mm}
Correspondingly, there is no parity equation that includes exactly one coded symbol among those indexed by $\tau$. Thus, if this set of coded symbols are hidden, there is no degree-1 parity equation to recover them. Since the  peeling decoder is essential for us to construct small incorrect-coding proof, the undecodable ratio $\alpha$ of a block is equivalent to the \emph{stopping ratio} of $\sH$, which is the size of the smallest stopping set divided by $n$.

\def\mJ{\boldsymbol J}


While CMT admits any erasure codes,  SPAR uses the method introduced in \cite{burshtein2004asymptotic,luby2001efficient} and analyzed in \cite{orlitsky2005stopping} for its proved ability to create, with high probability, parity matrices with a large stopping ratio. Given two integers $c$ and $d$ that satisfies $nc=(n-k)d$, we first generate an $nc\times(n-k)d$ permutation matrix $\mJ$ (a random row permutation of an $nc\times(n-k)d$ identity matrix). We then partition $\mJ$ into $n\times (n-k)$ slices, where each slice is a $c\times d$ sub-matrix. Then $\sH_{i,j}=1$ if and only if slice-$(i,j)$ contains an odd number of 1s, for $i\in[1:n]$ and $j\in[1:n-k]$. Such a random $\sH$ has the following three critical properties:
\begin{enumerate}
    \item It has a maximum row weight of $c$, and a maximum column weight of $d$;
    \item It has a non-zero probability to have a stopping ratio of at least $\alpha^*$, where $\alpha^*$ is a critical stopping ratio inherent to this method and is independent of $k$;
    \item It is NP-hard to find the minimum stopping set and determine the stopping ratio of $\sH$.
\end{enumerate}

Property 1 implies that the corresponding LDPC code has a maximum parity equation size of $d$. Property 2 implies that we could provide the same undecodable ratio (thus same sampling requirements) for all layers. Both are desirable.

Nevertheless, Property 2 and 3 together imply that we, as the developers, are not able to determine whether the LDPC codes we generate are good ($\alpha\geqslant \alpha^*$) or not, for any reasonably large $k$ (e.g., $k=1024$).

Fortunately, this problem can be easily solved through a \textbf{\em bad-code proof}. If an honest full node cannot fully decode the $k$ data symbols after receiving $(1-\alpha^*)n$ coded symbols, then this code is bad, and its small undecodable set has been found and hidden by a (very strong) malicious block producer. In this case, the honest full node can prove this code bad by broadcasting the indices of the $\alpha^*n$ coded symbols it is missing. Upon receiving and verify this bad-code proof, all the nodes in the system reject the associated block, and regenerate a code for the failed layer using an agreed random seed. This seed can be drawn from a pre-defined number sequence or the block header of a previous block, so that no consensus protocol is needed. Alternatively, distributed random number generation algorithms such as \cite{syta2017scalable} and \cite{bonneau2015bitcoin} can also be used for strictly unbiased randomness and consensus.

In other words, we solve the NP-hard problem of finding good codes by exploiting the computational resources of malicious party. Once it finds a small undecodable set and hides it, the system can easily detect this, reject the block, and update the code. This way, the system will settle at a good code for every layer eventually. As we will show in the next section, the probability of generating good codes is extremely high, so that SPAR can settle at good codes very quickly without having light nodes accept any fraud blocks. In addition, since bad code is a rare event, a heavy incentive/punishment scheme can be applied to deter false bad-code proof. Thus, the download and verification cost of bad-code proof is amortized to negligible throughout the course of the system.

%\vspace{-2mm}
%\begin{remark}
%The randomly generated $\sH$ may not directly admit a systematic code. More specifically, it may not be possible to convert $\sH$ to $\sH'=[\mathbf{P};\mathbf{I}_{n-k}]$ by just using column-wise eliminations. In this case, besides column-wise eliminations, row swap will be needed, and if $\sH$ is rank-deficient, extra linearly independent column(s) will be attached. Then one can use the resultant $\sH'$ for systematic encoding, and use a row-swapped version of $\sH$ for decoding, where the swapping is the same as those applied to obtain $\sH'$. This is a common practice in coding theory, and its detail is out of the scope of this paper.
%\end{remark}
%\vspace{-4mm}

\vspace{-4mm}
\subsection{Summary of the Actions of Different Node Types}
%\vspace{-6mm}
\begin{itemize}
\item \noindent {\bf Block producer (full node):} (a) It generates CMT and broadcasts the CMT root to all nodes, as well as broadcasts the entire original block (not CMT, as it can be retrieved using the original) to the full nodes only.  (b) On receiving sample requests from the light nodes, respond to them.

\item \noindent{\bf Light node:} (a) On receiving a new CMT root (or a CMT root of a pending block from a new full node), it makes separate, anonymous, and intermittent sampling requests with replacement to full nodes who claim that the block is available, as described in Section \ref{sec:samplingalgorithm}. (b) On receiving a sample, it broadcasts it to all connected full nodes. (c) If a node receives all requested samples, it assumes the block is available. (d) If a node does not receive all requested samples within a fixed time, it ``pends'' the block (i.e., keeps it in pending status). (e) If a node receives an incorrect-coding proof or bad-code proof, it rejects the block. In case of bad-code proof, it will also update the erasure code of the failed layer. 


%(b) If a sampling request is not responded by any full nodes, then it ``pends" the block (i.e., keeps the blocks status as pending). Otherwise, it will broadcast the received samples to full nodes. Finally, if it receives a valid incorrect-coding proof or bad-code proof, it will reject the block. 

\item \noindent{\bf Other full node.} (a) On receiving valid samples, it tries to recover the data block through both downloading the original data block from the other full nodes and collecting coded symbols forwarded by the light nodes. It will decode the tree from top to bottom using a hash-aware peeling decoder. (b) It rebroadcasts the received valid samples. (c) If an incorrect coding or a bad code has been detected, it will send the corresponding proof and reject this block. (d) If it has received/fully decoded a data block and verified it, it will declare the availability of this block to all other nodes and respond to sample requests from light nodes. 
\end{itemize}



